Tautological rings of Shimura varieties and cycle classes of Ekedahl-Oort strata

We define the tautological ring as the subring of the Chow ring of a Shimura variety generated by all Chern classes of all automorphic bundles. We explain its structure for the special fiber of a good reduction of a Shimura variety of Hodge type and show that it is generated by the cycle classes of the Ekedahl-Oort strata as a vector space. We compute these cycle classes. As applications we get the triviality of l-adic Chern classes of flat automorphic bundles in characterstic 0, an isomorphism of the tautological ring of smooth toroidal compactifications in positive characteristic with the rational cohomology ring of the compact dual of the hermitian domain given by the Shimura datum, and a new proof of Hirzebruch-Mumford proportionality for Shimura varieties of Hodge type.

==> Ch6CycleEO.tex <==
%=====================================================================

\section{Functoriality}

\subsection{Functoriality in the Zip Datum}\label{FuncZip}

To simplify notation it is often convenient for the computations in Subsection~\ref{HowCompute} to replace $G$ by some other group $\Gtilde$. Here we explain that this is harmless as long as $G$ and $\Gtilde$ have the same adjoint group.

Let $(G,\mu)$ and $(\Gtilde,\mgtilde)$ be two pairs consisting of a reductive group over $\BF_p$ and a cocharacter defined over the algebraic closure $k$ of $\BF_p$. Let
\[
f\colon G \to \Gtilde
\]
be a map of algebraic groups over $\FF_p$ with $f \circ \mu = \mgtilde$. Let $\kappa$ (resp.~$\kgtilde$) be the field of definition of the conjugacy class of $\mu$ (resp.~of $\mgtilde$). Then $\kgtilde \subseteq \kappa$.

Let $P$ and $Q$ be the parabolics and $E$ the zip group attached to $(G,\mu)$ as in Subsection~\ref{GZip}. Let $\Ptilde$, $\Qtilde$ and $\Etilde$ the parabolics and zip group attached similarly to $(\Gtilde,\mgtilde)$. Then $f$ induces maps $P \to \Ptilde$, $Q \to \Qtilde$, and $E \to \Etilde$ and hence a morphism
\[
[f]\colon \GZip^{\mu} \lto \GZip[\Gtilde]^{\mgtilde} \otimes_{\kgtilde} \kappa
\]
of algebraic stacks over $\kappa$.


\subsubsection*{Functoriality for maps inducing isomorphisms on the adjoint group}

\begin{lemma}\label{FunctorialityGZip}
Suppose that $f$ induces an isomorphism of the adjoint groups $G^{\rm ad} \iso \Gtilde^{\rm ad}$.
\begin{assertionlist}
\item\label{FunctorialityGZip1}
Let $\Ztilde$ be the radical of $\Gtilde$. Let $(T,B,z)$ be a frame as in Subsection~\ref{Frame} for $(G,\mu)$. Set $\Ttilde := \Ztilde f(T)$ and $\Btilde := \Ztilde f(B)$. Then $(\Ttilde, \Btilde, f(z))$ is a frame for $(\Gtilde,\mgtilde)$.
\item\label{FunctorialityGZip2}
The map $f$ induces an isomorphism $W \iso \Wtilde$ of the Weyl groups with their set of simple reflections attached to $(G,B,T)$ and $(\Gtilde,\Btilde,\Ttilde)$, respectively.
\item\label{FunctorialityGZip3}
The induced map $[f]$ is a homeomorphism of the underlying topological spaces.
\end{assertionlist} 
\end{lemma}

\begin{proof}
The hypothesis on $f$ means that $\Ker(f)$ is central and that $\Cent(\Gtilde)f(G) = \Gtilde$. As $\Ztilde f(G)$ is of finite index in $\Cent(\Gtilde)f(G)$ and $\Gtilde$ is connected, this implies $\Ztilde f(G) = \Gtilde$.
As $\Ztilde$ is a torus and clearly commutes with $f(T)$, $\Ttilde := \Ztilde f(T)$ is a torus. Its dimension is the reductive rank of $\Gtilde$. Hence it is a maximal torus. By hypothesis, $f$ induces a bijection between the roots of $(G,T)$ and of $(\Gtilde,\Ttilde)$. This shows that $\Ztilde f(B)$ is a Borel subgroup and that $f$ induces an isomorphism $W \iso \Wtilde$. This implies all remaining assertions. 
\end{proof}

We continue to assume that $f$ induces an isomorphism of the adjoint groups $G^{\rm ad} \iso \Gtilde^{\rm ad}$ and use the notation of the lemma. We identify $W$ with $\Wtilde$ via the isomorphism induced by $f$.

If we define $\GZipFlag[\Gtilde]^{\mgtilde}$ and $\Brh_{\Gtilde}$ using $(\Gtilde,\Ptilde,\Qtilde,\Btilde)$ then the key diagram \eqref{EqKey} and the corresponding diagram of Chow rings \eqref{EqKeyChow} is functorial for $f$. The induced map of $\BQ$-algebras $\Stilde \defeq \Sym(X^*(\Ttilde)_{\BQ}) \to S$ is equivariant for the action of $W$. More precisely, if we choose splittings of the exact sequences of tori
\begin{gather*}
1 \lto \Ker(f)^0 \lto T \lto T/\Ker(f)^0 \lto 1,\\
1 \lto f(T) \lto \Ttilde \lto \Ttilde/f(T) \lto 1,
\end{gather*}
then $\Stilde \to S$ is of the form
\[
\Stilde \epi \Sym(X^*(f(T))_{\BQ}) \liso \Sym(X^*(T/\Ker(f)^0)_{\BQ}) \mono S,
\]
where the second map is an isomorphism of $\BQ$-algebras with $W$-action. The map $\Stilde \to S$ is also equivariant for the action of the Frobenius because $f$ is defined over $\BF_p$.

\begin{proposition}\label{FuncChow}
Let $f\colon G \to \Gtilde$ be a map of algebraic groups defined over $\BF_p$ that induces an isomorphism on adjoint groups.
\begin{assertionlist}
\item\label{FuncChow1}
One has a commutative diagram of $\BQ$-linear maps
\begin{equation}\label{EqFuncPistar}
\begin{aligned}\xymatrix{
A^{\bullet}(\GZipFlag[\Gtilde]^{\mgtilde}) \ar[rr] \ar[d]_{\pi_*} & & A^{\bullet}(\GZipFlag^{\mu}) \ar[d]^{\pi_*} \\
A^{\bullet}(\GZip[\Gtilde]^{\mgtilde}) \ar[rr]^{\sim} & &  A^{\bullet}(\GZip^{\mu})
}\end{aligned}
\end{equation}
where the horizontal maps are the maps of $\BQ$-algebras induced by $f$. The lower horizontal map is an isomorphism.
\item\label{FuncChow2}
For $w \in {}^IW$ the numbers $\gamma(w)$ defined in Definition~\ref{DefGammaw} for $(G,\mu)$ coincide with those defined for $(\Gtilde,\mgtilde)$.
\end{assertionlist}
\end{proposition}

\begin{proof}
Under the identifications \eqref{ChowGZip1} and \eqref{ChowGZip2} the horizontal maps are both induced by the $W$-equivariant map $\Stilde \to S$. Hence the commutativity of \eqref{EqFuncPistar} follows from the concrete description of $\pi_*$ in Theorem~\ref{GysinFormula}. From Proposition~\ref{ChowGZipNaive} and Lemma~\ref{FunctorialityGZip}~\ref{FunctorialityGZip3} we also deduce that the lower horizontal map sends a $\BQ$-basis to a $\BQ$-basis. In particular it is an isomorphism.

Let us show \ref{FuncChow2}. The upper horizontal map sends for all $w \in W$ the cycle $[\bar{Z}^{\emptyset}_w]$ defined for $(\Gtilde,\mgtilde)$ to the cycle $[\bar{Z}^{\emptyset}_w]$ defined for $(G,\mu)$ because $\psi^*$ is functorial for $f$. Hence \ref{FuncChow2} follows from \ref{FuncChow1} and Proposition~\ref{ZwProjChow}.
\end{proof}



%---------------------------------------------------------------------

\subsection{Functoriality in the Shimura datum}




